Prior-Independent Mechanisms for Scheduling

We study the makespan minimization problem with unrelated selfish machines under the assumption that job sizes are stochastic. We design simple truthful mechanisms that under various distributional assumptions provide constant and sublogarithmic approximations to expected makespan. Our mechanisms are prior-independent in that they do not rely on knowledge of the job size distributions. Prior-independent approximation mechanisms have been previously studied for the objective of revenue maximization [Dhangwatnotai, Roughgarden and Yan'10, Devanur, Hartline, Karlin and Nguyen'11, Roughgarden, Talgam-Cohen and Yan'12]. In contrast to our results, in prior-free settings no truthful anonymous deterministic mechanism for the makespan objective can provide a sublinear approximation [Ashlagi, Dobzinski and Lavi'09].

==> old_macros.tex <==
\newcommand{\argmax}{\operatorname{argmax}}
\newcommand{\argmin}{\operatorname{argmin}}

\newcommand{\poly}{{\text {poly }}}


\newcommand{\groundset}{J}


\newcommand{\A}{{\mathcal A}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\iid}{{i.~i.~d.\ }}

\newcommand{\val}{v}
\newcommand{\vals}{{\mathbf \val}}
\newcommand{\valsmi}{{\mathbf \val}_{-i}}
\newcommand{\vali}[1][i]{{\val_{#1}}}
\newcommand{\valj}[1][j]{{\val_{#1}}}


\newcommand{\partition}{J}
%\newcommand{\parts}{{\mathbf \partition}}
\newcommand{\parts}{\Pi}
\newcommand{\parti}[1][i]{{\partition_{#1}}}


\newcommand{\bid}{b}
\newcommand{\bids}{{\mathbf \bid}}
\newcommand{\bidi}[1][i]{{\bid_{#1}}}

\newcommand{\virt}{\phi}
\newcommand{\virts}{{\mathbf \virt}}
\newcommand{\virti}[1][i]{{\virt_{#1}}}

\newcommand{\virtinv}{\virt^{-1}}
\newcommand{\virtiinv}[1][i]{\virt_{#1}^{-1}}
\newcommand{\virtval}{\nu}

\newcommand{\ivirt}{\bar{\virt}}
\newcommand{\ivirtinv}{\ivirt^{-1}}
\newcommand{\ivirtiinv}{\ivirt_i^{-1}}
\newcommand{\ivirti}[1][i]{{\ivirt_{#1}}}

\newcommand{\vmin}{\ell}
\newcommand{\vmax}{h}

\newcommand{\dist}{F}
\newcommand{\dists}{{\mathbf \dist}}
\newcommand{\disti}[1][i]{{\dist_{#1}}}
\newcommand{\distj}[1][j]{{\dist_{#1}}}

\newcommand{\dens}{f}
\newcommand{\denss}{{\mathbf \dens}}
\newcommand{\densi}[1][i]{{\dens_{#1}}}
\newcommand{\densj}[1][j]{{\dens_{#1}}}

\newcommand{\price}{p}
\newcommand{\prices}{{\mathbf \price}}
\newcommand{\pricei}[1][i]{{\price_{#1}}}
\newcommand{\pricej}[1][j]{{\price_{#1}}}
\newcommand{\pricemi}[1][i]{{\price^M_{#1}}}
\newcommand{\pricemj}[1][j]{{\price^M_{#1}}}
\newcommand{\pricesi}[1][i]{{\price^S_{#1}}}
\newcommand{\rightpeakpricei}{\overline{\pricei}}
\newcommand{\leftpeakpricei}{\underline{\pricei}}

\newcommand{\rprice}{p}
\newcommand{\rprices}{{\mathbf \rprice}}
\newcommand{\rpricei}[1][i]{{\rprice_{#1}}}

\newcommand{\prob}{q}
\newcommand{\probs}{{\mathbf \prob}}
\newcommand{\probi}[1][i]{{\prob_{#1}}}
\newcommand{\probj}[1][j]{{\prob_{#1}}}
\newcommand{\probmi}[1][i]{{\prob^M_{#1}}}
\newcommand{\probmj}[1][j]{{\prob^M_{#1}}}
\newcommand{\probsi}[1][i]{{\prob^S_{#1}}}
\newcommand{\rightpeakprobi}{\overline{\probi}}
\newcommand{\leftpeakprobi}{\underline{\probi}}

\newcommand{\expect}{\mathop{\operatorname{E}}}
\newcommand{\pr}{\mathop{\operatorname{Pr}}}

\newcommand{\Mye}{\mathcal M}
\newcommand{\gMye}{{\mathcal M}^{G}} 
\newcommand{\Alg}{\mathcal A}
\newcommand{\biopt}{\mathrm{OPT}_{n/2}} %bi-criteria OPT
\newcommand{\ziconst}{d} % constant associated with the random variable Z_i
\newcommand{\ticonst}{k_1} % constant arising when bounding E[max_i t_i] by OPT_{n/2}
\newcommand{\exziconst}{2c} % constant denoting the expectation of Z_i; was k_2
\newcommand{\finaliidconst}{k} % final constant of approximation for iid case

\newcommand{\VCGc}{\ensuremath{\mathrm{VCG}_c}}
\newcommand{\OPT}{{\mbox {OPT}}}
\newcommand{\wel}{{\mbox {WEL}}}
\newcommand{\OPTh}{\ensuremath{\mathrm{OPT}_{1/2}}}
\newcommand{\welh}{\ensuremath{\mathrm{WEL}_{1/2}}}
%\newcommand{\OPT}{\ensuremath{\mathrm{OPT}}}
\newcommand{\hyb}{\ensuremath{\mathrm{HYB}}}
\newcommand{\msp}{\textbf{msp}}

\newcommand{\rt}{r}
\newcommand{\rti}[1][i]{\rt_{#1}}
\newcommand{\rtji}[1][j]{{\rt_{#1i}}}
\newcommand{\rts}{\mathbf r}
\newcommand{\Rt}{\mathcal R}
\newcommand{\Rti}[1][i]{{\mathcal \Rt_{#1}}}

\newcommand{\ex}{\mathop{\operatorname{E}}}

\newcommand{\out}{x}
\newcommand{\Out}{\mathcal X}

\newcommand{\mech}{\mathcal M}

\newcommand{\al}{\mathcal{A}}

\newcommand{\Tij}[1][j]{{T_{i,#1}}}
\newcommand{\Bi}{{B_i}}
\newcommand{\dmax}[1]{\max_{#1 \text{ draws}}}

\newcommand{\G}{\mathcal{G}}
\newcommand{\B}{\mathcal{B}}



==> related.tex <==
\subsection*{Related work}

% In their seminal paper introducing algorithmic mechanism design, Nisan and
% Ronen~\cite{NR99} presented makespan minimization as an example of an objective
% that seems inherently at odds with incentive constraints. They presented an
% $m$-approximation to makespan as well as a lower bound of $2$ on the
% approximation factor for deterministic mechanisms. 

Following the work of Nisan and Ronen~\cite{NR99}, a series of papers
presented better lower bounds for deterministic as well as randomized
mechanisms~\cite{ADL09, CKV07, CKK07, KV07, MS07}. Given the
difficulty of the general multi-parameter problem, several special
cases have also been explored.  These include: (1) the related
machines setting~\cite{AT01, DDDR08} where every machine has a single
private parameter, namely its speed, (2) the special case of two
machines~\cite{DS08, CKV08, LY08, LY08-2, Lu09}, and, (3) the special
case where job sizes take on only two possible values, high and
low~\cite{LS07}.  All of this work is in the prior free setting. In
the Bayesian setting, Chawla, Immorlica and Lucier~\cite{CIL12}
recently showed that the makespan objective does not admit black-box
reductions from incentive compatible mechanisms to approximation
algorithms in the same way as, for example, social welfare
maximization \cite{HL10}.

A growing literature addresses approximation in Bayesian mechanism
design for objectives such as welfare and revenue.  Simple
approximately optimal auctions for the revenue objective in settings
with single-dimensional agent preferences were considered by Hartline
and Roughgarden~\cite{HR09}.  Dhangwatnotai, Roughgarden, and
Yan~\cite{DRY10} extend this work to design prior independence
mechanisms for the same setting.  These approaches were generalized to
(multi-dimensional) multi-item auctions by~\cite{DHKN11, RTY12} using
an analysis approach from \cite{CHK07,CHMS10}.  Importantly, the mechanism of
\cite{RTY12} is a ``supply limiting'' mechanism which is conceptually
very similar to our restriction of the number of jobs each machine is
allowed to process.  In this line of work non-linear objectives such
as makespan are a significant departure from linear objectives such as
revenue.

